AI for the Open-World: the Learning Principles

During the past decades, numerous successes of AI has been made on "specific capabilities", named closed-world, such as artificial environments or specific real-world tasks. This well-defined narrow capability brings two nice benefits, a clear criterion of success and the opportunity to collect a lot of examples. The criteria not only reveal whether a machine has achieved a goal, but reveal how the machine falls short of the goal. As a result, human designers can fix the problems one after the other until the machine is deemed good enough for the task. Furthermore, the large set of collected examples reduces the difficulty of this problem-fixing process (by the central limit theorem). Do the success in closed-world translate into broad open-world, where a machine is required to perform any task that a human could possibly undertake with fewer examples and less priori knowledge from human designers? No. Because competence in a specific task provides little insight in handling other tasks, the valuable criteria for specific tasks become helpless when handling broader unseen tasks. Furthermore, due to the shortage of examples in unseen tasks, central limit theorem does not stand on our side. At the end, human designers lose the oscilloscope to "hack" an AI system for the open-world. Achieving AI for the open-world requires unique learning principles and innovated techniques, which are different from the ones in building AI for the closed-world. This thesis explores necessary learning principles required to construct AI for the open-world, including rich features (analogy a large tool box), disentangled representation (an organized tool box), and inference-time learning (a tool-savvy hand). Driven by the learning principles, this thesis further proposes techniques to use the learning principles, conducts enormous large-scale experiments to verify the learning principles.

==> bonsai_method.tex <==
\subsection{Bonsai: Adversarially creating orthogonal learning signals}
\label{sec:rfc}

This section presents tools for constructing rich representations. First, we describe a mathematically sound approach to the problem of constructing a rich set of diverse features and we introduce the notions of \emph{discovery} and \emph{synthesis} episodes. Then we show how to use Distributionally Robust Optimization (DRO) to cut on the synthesis episodes. Finally, we present a practical Bonsai algorithm.

\subsubsection{Feature discovery}

Intuitively, constructing additional features is desirable when using these features increases the system performance on a pertinent subset of examples. Best would of course achieve a large performance increase on large subsets of examples.

For the purposes of this section, let $\Phi_k(x)$ be a large vector containing all previously constructed $k$ features for pattern $x$. Our first step consists of defining an ensemble $P=\{D^1\dots{D^i}\dots\}$ of pertinent subsets $D^i$ of the training set. An effective way to choose a good ensemble of subsets is discussed at the end of this section. Having defined such subsets, we can define costs $C_i(\Phi,w)$ that measure
the quality of a feature set $\Phi$ measured on subset $D^i$:
\[
   C_i(\Phi,w) = \frac{1}{|D^i|} \sum_{(x,y)\in D^i} \ell(y, w^\top \Phi(x))
\]
where $w$ represent the weights of a linear layer and $\ell(y,\hat{y})$ is a convex loss. In the context of deep learning, considering a linear layer operating a large feature vector is not an unreasonable way to investigate the effectiveness of a representation \citep{ntk}. We can reweigh the training data in a manner that emphasizes the weaknesses of our current set of features, that is,
\begin{equation}
    \label{eq:r-rw}
    R_{rw} = \max_\lambda \min_w \sum_i \lambda_i C_i(\Phi_k,w)
\end{equation}
where the $\lambda_i$ coefficients are positive and sum to 1.  Let $\lambda^*_i$ be the pessimal mixture coefficients resulting from
optimization problem~\eqref{eq:r-rw}.  We can then learn a new set of features that help performance on this pessimal mixture,
\begin{equation}
    \label{eq:rprime-rw}
    R'_{rw} = \min_{w,\Phi} \sum_i \lambda^*_i C_i(\Phi,w)~.
\end{equation}
The main difference is that we are now training the features, yielding a new feature vectors $\Phi^*(x)$. If $R'_{rw}$  \eqref{eq:rprime-rw} is smaller than $R_{rw}$ \eqref{eq:r-rw}, then we know that $\Phi^*$ contains \emph{new useful features that were not present} in $\Phi_k$. This is the \emph{discovery phase}.

The next step consists in forming new feature vectors $\Phi_{k+1}(x)$ that contain the features present in both $\Phi_k$ and $\Phi^*$, a \emph{synthesis phase}. We can then iterate and obtain additional useful and diverse features at each iteration. The synthesis phase can be as simple as a vector concatenation. In the context of deep learning, however, one often has to use distillation, as discussed later in section~\ref{sec:rfc}.

The selection of a pertinent ensemble of subsets certainly affects which new features will be constructed at each iteration. In particular, it is desirable to make $R_{rw}$ as high as possible using a minimal number of subsets. This goal can be easily achieved by forming subsets containing examples that were either correctly classified or misclassified by the learning systems constructed by problem \eqref{eq:rprime-rw}.


\subsubsection{Using DRO}

We now show how a DRO reformulation of this process can cut the intermediate synthesis phase. Because the $C_i$ are convex in $w$,
we can first apply von Neumann's minimax theorem \citep[theorem~3]{simons1995} to problem \eqref{eq:r-rw} and obtain a DRO problem \citep{Ben-TalGN09}:
\begin{multline}
\label{eq:r-dro}
 R_{rw} ~=~ \max_\lambda \min_w \sum_i \lambda_i C_i(\Phi_k,w) 
        = \min_w \max_\lambda \sum_i \lambda_i C_i(\Phi_k,w) 
        = \min_w \max_i C_i(\Phi_k,w) ~=~  R_{dro}~. 
\end{multline}
The next step is to run this same DRO optimization while also learning the features
\begin{equation}
    \label{eq:rprime-dro}
    R'_{dro} = \min_{w,\Phi} \max_i C_i(\Phi,w)~.
\end{equation}
To understand how quantity $R'_{dro}$ relates to $R'_{rw}$, we can use the max-min inequality as follows:
\begin{multline*}
  R'_{dro} = \min_{w,\Phi} \max_\lambda \sum_i\lambda_i C_i(\Phi,w) 
    \ge \max_\lambda \min_{w,\Phi} \sum_i \lambda_i C_i(\Phi,w) 
    \ge \min_{w,\Phi} \sum_i \lambda^*_i C_i(\Phi,w) = R'_{rw}~.
\end{multline*}
In other words, if $R'_{dro}$ is smaller than $R_{dro}$, then $R'_{rw}$ is smaller than $R_{rw}=R_{dro}$, and the new feature vector $\Phi$ contains new and useful features. The advantage of this approach is that
problem \eqref{eq:rprime-dro} does not involve mixture coefficients $\lambda^*$. Therefore there is no need to solve \eqref{eq:r-dro} or \eqref{eq:r-rw}, and no need for a synthesis phase at each iteration. The synthesis phase is only needed to construct the final rich representation after the last iteration.


\subsubsection{The practical Bonsai algorithm}

We now describe a practical algorithm that implements the ideas discussed in the previous subsection in a manner that is usable with ordinary deep networks. 
The workhorse of this algorithm is the Robust Empirical Risk Minimisation (RERM) algorithm (Algorithm~\ref{alg:rerm}) which takes an ensemble of datasets $D^k$ representing multiple distributions and seeks neural network weights that simultaneously yields small errors for all these distributions. RERM is in fact a minimal form of DRO with overfitting control by cross-validation.


\begin{algorithm}[ht]
\caption{Robust Empirical Risk Minimization (RERM)}
\label{alg:rerm}
\begin{algorithmic}[1]
\STATE  \textbf{Required:} datasets $D^k = \{(x^k_i, y^k_i)\}_{i=1}^{n^k}$, for $k = 1, \ldots, N$; model $f$; learning rate $\alpha$
\STATE  Randomly initialize $f$
\WHILE[ \texttt{  // By validation}]{no overfit}
\STATE  Train on  datasets $D^1,\ldots,D^N$ by DRO: $f \leftarrow f - \alpha \cdot \nabla_f \left[\max_k \left(\frac{1}{|D^k|} \sum_{(x^k_i, y^k_i) \in D^k} \ell(f(x^k_i), y^k_i)\right)_{k=1}^N\right]$
\ENDWHILE
\STATE \textbf{return} $f$
\end{algorithmic}
\end{algorithm}

The Bonsai algorithm (Algorithm~\ref{alg:rich_feature}) first performs a predefined number of \emph{discovery episodes}, using RERM to repeatedly solve an analogue of problem \eqref{eq:rprime-dro} that constructs a model $f_k$ at each iteration, using an ensemble of subsets formed by selecting which examples were correctly or incorrectly recognized by the models $f_0\dots f_{k-1}$ constructed during the previous iterations.

The Bonsai algorithm performs a distillation-based \emph{synthesis episode}. The goal is to learn a representation network $\Phi(x)$ such that we can emulate the functions $f_k$ using a simple network with weights $w_k$ on top of $\Phi(x)$. To that effect, we use the $f_k$ models to compute pseudo-labels $y^k(x)$ for each example $x$. We then train a composite model with parameters $\Phi$, $w_1$, \dots, $w_K$ whose $k$ outputs are trained to replicate the pseudo-labels.

\par\noindent
\emph{Why use linear classifiers in synthesis episode (line 11)?}
\par
The goal is to perform the synthesis step by distillation into a network whose architecture is as close as possible as the architecture of the “source” networks. However the distillation network needs one head for each source network. The least intrusive way to implement multiple heads is to duplicate the very last layer, hence linear. The opposite approach would be to claim the whole network is a classifier and the feature extractor is the identity. In this case, we can get a perfect synthesis loss (Alg \ref{alg:rich_feature}, line 14) with an identity feature extractor which is obviously useless. We leave the non-linear classifier in \emph{synthesis phase} as a future work. 

\par\noindent
\emph{What if the first RERM round achieves zero errors (line~3)?}
\par
The training set of the first RERM round is the union of the data associated with all OOD training environments. Since RERM avoids overfitting using a validation set (Alg \ref{alg:rerm}, line 3), a perfect accuracy on both the merged training and validation sets means that the features discovered in the first round are already invariant in all training environments and perfectly predictive (100\% accuracy). Therefore no further rounds are necessary since we already have a solution. This is in fact a degeneracy of the invariant training concept.

\begin{algorithm}[t]
\caption{Bonsai algorithm (RFC)}
\label{alg:rich_feature}
\begin{algorithmic}[1]
\STATE \textbf{Input:} dataset $D$; the number of discovering rounds $K$
\STATE \texttt{// Discovery episodes}
\STATE $f_1 \leftarrow \text{RERM}(\{D\})$ 
\STATE Split $D$ into groups $A_1,B_1$ according to $f_1$. ($A_1=$ examples correctly classified by $f_1$, $B_1 = D \backslash A_1$)   
\STATE Available groups $P = \{A_1,B_1\}$
\FOR{$k \in [2,\ldots, K]$}
\STATE $f_k \leftarrow \text{RERM}(P)$
\STATE Split $D$ into groups $A_k,B_k$ according to $f_k$
\STATE $P \leftarrow P \cup \{A_k, B_k\}$
\ENDFOR
\STATE \texttt{// Synthesis episode}
\STATE Pick a feature extractor function $\Phi$, and $K$ linear classifiers $\omega_1,...\omega_k$ at random
\STATE Create $K$ groups of pseudo-labels ${y}^k$ by applying each $f_k$ on $D$ 
\STATE $A = A_i \cap ... \cap A_K$
\STATE Update $\Phi, \omega$ such that each pseudo-label ${y}^k$ is well learned by the corresponding classifier $\omega_k$ and $\Phi$: 
$\sum_{k=1}^{K} \frac{1}{|{A}|}\sum_{(x_i,{y}_i^k)\in {A}}\ell(\omega_k  \circ \Phi(x_i), {y}^k_i) + \frac{1}{|D\backslash {A}|}\sum_{(x_i,{y}_i^k)\notin {A}} \ell(\omega_k  \circ \Phi(x_i), {y}^k_i)$
\STATE \textbf{return} $\Phi, \{\omega_k\}_{k=1}^K$

\end{algorithmic}
\end{algorithm}



==> defs.tex <==

\usepackage{graphicx} %


\usepackage{amsthm} %
\usepackage{amsmath} %

\usepackage{amsfonts}
\usepackage{amssymb}

\RequirePackage[T1]{fontenc}
\ifxetex
  \RequirePackage[tt=false]{libertine}
\else
  \RequirePackage[tt=false, type1=true]{libertine}
\fi
\RequirePackage[varqu]{zi4}
\RequirePackage[libertine]{newtxmath}


\usepackage{mathpartir}
\newcommand{\bmmax}{2}
\usepackage{bm}



\usepackage{booktabs}   %
\usepackage[labelformat=simple]{subcaption} %
\renewcommand\thesubfigure{(\alph{subfigure})}

\usepackage[T1]{fontenc} %
\usepackage[utf8]{inputenc} %

\usepackage{amssymb}

\usepackage[final]{listings}
\lstset{mathescape=true}


\usepackage{tikz}
\usetikzlibrary{matrix,arrows,positioning,calc,fit,backgrounds}

\usepackage[shortlabels, inline]{enumitem}
\makeatletter
\newcommand{\myitem}[1][]{
  \protected@edef\@currentlabel{#1}%
\item[#1]
}
\makeatother

\usepackage{mathtools}

\usepackage{etoolbox}

\usepackage{array}
\newcolumntype{L}{>$l<$}

\usepackage{stmaryrd}

\usepackage{dashbox}

\usepackage{scalerel}

\usepackage{mathpartir}

\usepackage{xspace}
\usepackage{multirow}

\usepackage{breakcites}

\usepackage{natbib}
\setcitestyle{%
    authoryear,%
    open={[},close={]},citesep={;},%
    aysep={},yysep={,},%
    notesep={, }}
\let\cite\citep

\usepackage[toc,page]{appendix}
\usepackage{tablefootnote}




\newcommand\blfootnote[1]{%
  \begingroup
  \renewcommand\thefootnote{}\footnote{#1}%
  \addtocounter{footnote}{-1}%
  \endgroup
}

\renewcommand{\le}{\leqslant}
\renewcommand{\ge}{\geqslant}

\newcommand{\R}{\ensuremath{\mathbb{R}}}
\newcommand{\Q}{\ensuremath{\mathbb{Q}}}
\newcommand{\Z}{\ensuremath{\mathbb{Z}}}
\newcommand{\N}{\ensuremath{\mathbb{N}}}
\newcommand{\T}{\ensuremath{\mathbb{T}}}
\newcommand{\C}{\ensuremath{\mathbb{C}}}

\newcommand{\eps}{\varepsilon}
\newcommand{\closure}[1]{\ensuremath{\overline{#1}}}

\newcommand{\Land}{\bigwedge}
\newcommand{\Lor}{\bigvee}
\newcommand{\es}{\emptyset}
\newcommand{\incl}{\subseteq}
\newcommand{\impl}{\Rightarrow}
\renewcommand{\iff}{\Leftrightarrow}
\newcommand{\ra}{\rightarrow}
\newcommand{\sat}{\vDash}
\newcommand{\notsat}{\nvDash}
\newcommand{\proves}{\vdash}
\newcommand{\provesIff}{\mathrel{\dashv\vdash}}
\newcommand{\boolTrue}{\top}
\newcommand{\boolFalse}{\bot}

\newcommand{\dom}{\operatorname{\mathsf{dom}}}
\newcommand{\range}{\operatorname{\mathsf{rng}}}
\newcommand{\restrict}[2]{{#1}|_{#2}}
\newcommand{\pto}{\rightharpoonup}

\newcommand{\defeq}{\coloneqq}
\newcommand{\defiff}{\vcentcolon\iff}

\newcommand{\pipe}{\triangleright}

\newcommand{\Aa}{{\mathcal{A}}}
\newcommand{\Bb}{{\mathcal{B}}}
\newcommand{\Cc}{{\mathcal{C}}}
\newcommand{\Dd}{{\mathcal{D}}}
\newcommand{\Ee}{{\mathcal{E}}}
\newcommand{\Ff}{{\mathcal{F}}}
\newcommand{\Gg}{{\mathcal{G}}}
\newcommand{\Hh}{{\mathcal{H}}}
\newcommand{\Ii}{{\mathcal{I}}}
\newcommand{\Jj}{{\mathcal{J}}}
\newcommand{\Kk}{{\mathcal{K}}}
\newcommand{\Ll}{{\mathcal{L}}}
\newcommand{\Mm}{{\mathcal{M}}}
\newcommand{\Nn}{{\mathcal{N}}}
\newcommand{\Oo}{{\mathcal{O}}}
\newcommand{\Pp}{{\mathcal{P}}}
\newcommand{\Qq}{{\mathcal{Q}}}
\newcommand{\Rr}{{\mathcal{R}}}
\newcommand{\Ss}{{\mathcal{S}}}
\newcommand{\Tt}{{\mathcal{T}}}
\newcommand{\Uu}{{\mathcal{U}}}
\newcommand{\Vv}{{\mathcal{V}}}
\newcommand{\Ww}{{\mathcal{W}}}
\newcommand{\Yy}{{\mathcal{Y}}}
\newcommand{\Zz}{{\mathcal{Z}}}

\newcommand{\paren} [1] {\ensuremath{ \left( {#1} \right) }}
\newcommand{\bigparen} [1] {\ensuremath{ \Big( {#1} \Big) }}
\newcommand{\tuple}[1]{\ensuremath{\langle #1 \rangle}}
\newcommand{\abs}[1]{\ensuremath{\lvert #1 \rvert}}
\newcommand{\setcomp}[2]{\ensuremath{\left\{#1\;\middle|\;#2\right\}}}

\newcommand{\refCh}[1]{Chapter~\ref{#1}}
\newcommand{\refSc}[1]{Section~\ref{#1}}
\newcommand{\refFig}[1]{Figure~\ref{#1}}
\newcommand{\refDef}[1]{Definition~\ref{#1}}
\newcommand{\refLem}[1]{Lemma~\ref{#1}}
\newcommand{\refThm}[1]{Theorem~\ref{#1}}
\newcommand{\refAlg}[1]{Algorithm~\ref{#1}}
\newcommand{\refEx}[1]{Example~\ref{#1}}
\newcommand{\refCor}[1]{Corollary~\ref{#1}}
\newcommand{\refTab}[1]{Table~\ref{#1}}
\newcommand{\refEq}[1]{\ensuremath{(\ref{#1})}}
\newcommand{\refRule}[1]{(\ref{#1})}
\newcommand{\refApp}[1]{Appendix~\ref{#1}}

\newcommand{\tool}[1]{\textsf{#1}}
\newcommand{\code}[1]{\textnormal{\small\texttt{#1}}}


\newcommand{\tick}{\ensuremath{\checkmark}}
\newcommand{\cross}{\text{\sffamily X}}





\DeclareMathOperator*{\argmin}{argmin} %
\DeclareMathOperator{\argmininline}{argmin} 
\DeclareMathOperator*{\argmax}{argmax} %
\DeclareMathOperator{\argmaxinline}{argmax}


\newcommand{\bfparagraph}[1]{\paragraph{\textbf{#1}}}
\def\R{\mathbb{R}}
\def\E{\mathbb{E}}
\def\w{\mathbf{w}}
\usepackage{makecell}
\usepackage{xcolor,colortbl}
\def\argmin{\mathop{\rm arg\,min}}
\def\argmax{\mathop{\rm arg\,max}}
\def\calD{\ensuremath{{\cal D}}} %
\def\calL{\ensuremath{{\cal L}}} %
\def\calN{\ensuremath{{\cal N}}} %
\def\R{\mathbb{R}}
\def\E{\mathbb{E}}
\def\w{\mathbf{w}}


\def\synthdistill{\textsc{Distill}}  %
\def\synthcat{\textsc{Cat}}    %

\def\plotlabel#1{\textsf{\small``#1''}}

\long\def\TODO#1{\textcolor{red}{TODO:#1}}
\def\eg.{\mbox{e.}\mbox{g.}}
\def\ie.{\mbox{i.}\mbox{e.}}

\def\eg.{\mbox{e.}\mbox{g.}}
\def\ie.{\mbox{i.}\mbox{e.}}
\def\R{\mathbb{R}}
\def\E{\mathbb{E}}
\def\xbar{\Bar{x}}
\def\ttop{{\!\top}}
\def\w{{\mathbf{w}}}
\def\babistories{\textsc{BabiStories}}
\contourlength{1pt} %
\contournumber{10} %
\definecolor{teal1}{HTML}{b5d1ae}
\definecolor{teal2}{HTML}{80ae9a}
\definecolor{teal3}{HTML}{568b87}
\definecolor{teal4}{HTML}{326b77}
\definecolor{teal5}{HTML}{1b485e}
\definecolor{teal6}{HTML}{122740}
\definecolor{darkred}{HTML}{ae282c}
\definecolor{red}{HTML}{e02b35}
\definecolor{medred}{HTML}{d47264}
\definecolor{darkblue}{HTML}{2066a8}
\definecolor{blue}{HTML}{1a80bb}
\definecolor{medblue}{HTML}{3594cc}
\definecolor{lightblue}{HTML}{8cc5e3}
\usepackage{pifont}

\definecolor{main}{HTML}{5989cf}    %
\definecolor{sub}{HTML}{cde4ff}     %

\newtcolorbox{boxA}{
    boxrule = 1.5pt,
    colframe = black %
}

\newtcolorbox{boxB}{
    fontupper = \bf\color{main}, %
    boxrule = 1.5pt,
    colframe = main,
    rounded corners,
    arc = 5pt   %
}

\newtcolorbox{boxC}{
    colback = sub, %
    boxrule = 0pt  %
}

\newtcolorbox{boxD}{
    colback = sub, 
    colframe = main, 
    boxrule = 0pt, 
    toprule = 3pt, %
    bottomrule = 3pt %
}

\newtcolorbox{boxE}{
    enhanced, %
    boxrule = 0pt, %
    borderline = {0.75pt}{0pt}{main}, %
    borderline = {0.75pt}{2pt}{sub} %
}

\newtcolorbox{boxF}{
    fontupper = \bf,
    colback = sub,
    enhanced,
    boxrule = 1.5pt, 
    colframe = white, %
    borderline = {1.5pt}{0pt}{main, dashed} %
}

\newtcolorbox{boxG}{
    enhanced,
    boxrule = 0pt,
    colback = sub,
    borderline west = {1pt}{0pt}{main}, 
    borderline west = {0.75pt}{2pt}{main}, 
    borderline east = {1pt}{0pt}{main}, 
    borderline east = {0.75pt}{2pt}{main}
}

\newtcolorbox{boxH}{
    colback = sub, 
    colframe = main, 
    boxrule = 0pt, 
    leftrule = 6pt %
}

\newtcolorbox{boxI}{
    colback = sub, 
    colframe = main, 
    boxrule = 0pt, 
    toprule = 6pt %
}

\newtcolorbox{boxJ}{
    sharpish corners, %
    colback = sub, 
    colframe = main, 
    boxrule = 0pt, 
    toprule = 4.5pt, %
    enhanced,
    fuzzy shadow = {0pt}{-2pt}{-0.5pt}{0.5pt}{black!35} %
}

\newtcolorbox{boxK}{
    sharpish corners, %
    boxrule = 0pt,
    toprule = 4.5pt, %
    enhanced,
    fuzzy shadow = {0pt}{-2pt}{-0.5pt}{0.5pt}{black!35} %
}

\newtcolorbox{boxL}{
    fontupper = \color{main},
    rounded corners,
    arc = 6pt,
    colback = sub, 
    colframe = main!50, 
    boxrule = 0pt, 
    bottomrule = 4.5pt 
}

\newtcolorbox{boxM}{
    fontupper = \color{white},
    rounded corners,
    arc = 6pt,
    colback = main!80, 
    colframe = main, 
    boxrule = 0pt, 
    bottomrule = 4.5pt,
    enhanced,
    fuzzy shadow = {0pt}{-3pt}{-0.5pt}{0.5pt}{black!35}
}

\providecommand{\keywords}[1]
{
  \small	
  \textbf{\textit{Keywords---}} #1
}


==> randomness_method.tex <==


This section investigates the effect of concatenating representations obtained by multiple training episodes that only differ by their random seed. 

Despite the \emph{intentional lack of diversity} of these ensembles, the performance improvements observed on tasks involving distribution changes are far greater than the in-distribution performance improvements. This proves that representations constructed by multiple training episodes are indeed different. Even though their concatenation carries little additional information for in-distribution, these experiments show how they become substantially more informative when tasks
or distributions change. 

Meanwhile, we obtain worse performance (a) when we train a network whose size matches that of the ensemble from scratch, or (b) when we fine-tune the concatenated representations in a single additional run. We contend that this happens because optimization inherently impoverishes the representations in a manner that makes sense in-distribution but hurts out-of-distribution, and we propose \emph{two-stage fine-tuning} (Figure~\ref{fig:twostageft}) to correct this behavior.
 \begin{figure}[t]
\centering
\includegraphics[height=0.24\linewidth]{art/2stagefinetune.pdf}
\caption{\emph{Two-stage fine-tuning} consists of fine-tuning each network separately, then concatenating their feature extractors, now frozen, and training a final classifier. }
\label{fig:twostageft}
\end{figure}

